Mitigating Bias in Facial Analysis Systems by Incorporating Label Diversity

Facial analysis models are increasingly applied in real-world applications that have significant impact on peoples' lives. However, as literature has shown, models that automatically classify facial attributes might exhibit algorithmic discrimination behavior with respect to protected groups, potentially posing negative impacts on individuals and society. It is therefore critical to develop techniques that can mitigate unintended biases in facial classifiers. Hence, in this work, we introduce a novel learning method that combines both subjective human-based labels and objective annotations based on mathematical definitions of facial traits. Specifically, we generate new objective annotations from two large-scale human-annotated dataset, each capturing a different perspective of the analyzed facial trait. We then propose an ensemble learning method, which combines individual models trained on different types of annotations. We provide an in-depth analysis of the annotation procedure as well as the datasets distribution. Moreover, we empirically demonstrate that, by incorporating label diversity, our method successfully mitigates unintended biases, while maintaining significant accuracy on the downstream tasks.

==> sections/3_preliminary.tex <==
% \section{Preliminary}
% \label{sec:preliminary}

% In this section, we describe preliminary information which is useful for the deep understanding of our work.
% We start by formalizing the notation applied in this work.
% We then introduce the evaluation metrics used to assess our models.
% Finally, we describe the dataset used to train and evaluate our models.

% \subsection{Notation}
% \label{subsec:notation}

% We define a dataset $D$ consisting of $D = (S, X, Y)$, where $S$ represents sensitive attributes such as gender and age, $X$ represents features, and $Y$ represents the annotated ground-truth labels.
% We suppose there are $N$ samples in total and we use $S_i$, $X_i$, $Y_i$ to represent the features of $i$-th sample.
% To simplify, we suppose the sensitive attribute $S$ and the outcome $Y$ are binary, which means $Y, S = \{0, 1\}$. We set $S = 1$ as the privileged group and $Y = 1$ as the favored outcome.
% In order to train a machine learning model on dataset $D$, one must optimize parameters $\theta$ of function $f_\theta: X \rightarrow \R^{|Y|}$ to produce accurate predictions.
% In this work, we minimize the standard cross-entropy loss $L$ over dataset $D$ to provide the correct prediction $\hat{Y}$.
% A fair machine learning problem is to design a fair predictor $\hat{Y}$
% with parameters $\theta$ : $X \times S \rightarrow Y$, which maximizes the likelihood $P(Y, X, S | \theta)$ while satisfying some specific fair constraints, which we will introduce in the next section.

% \subsection{Evaluation Metric}
% \label{subsec:eval_metric}

% Several different metrics~\cite{barocas2016big, berk2018fairness, chouldechova2017fair, hardt2016equality, kleinberg2016inherent} have been proposed to mathematically measure and represent bias, fairness and/or discrimination of machine learning models. 
% Although the literature has defined a myriad of notions to quantify fairness notions, each one has different aspects of what is be considered ``fair''. 
% This is mainly a consequence of having various different interpretations of what means for an algorithm to be considered ``fair''.
% The fairness notions may be sub-divided into two different views: \textit{individual fairness}, which argues that similar individuals (inputs) should yield similar predictions (output); and \textit{group fairness}, which defends that instances should be grouped according to a specific sensitive attribute.

% Most quantitative definitions and measures of fairness are centered around three fundamental aspects of a (binary) classifier~\cite{caton2020fairness}: 
% First, the sensitive variable $S$ that defines the groups (for group fairness) or individual attributes (for individual fairness) for which we want to measure fairness. 
% Second, the target variable $Y$, which has, in binary classification scenario, two possible values ($Y=0$ or $Y=1$). 
% Third, the classification score $P$, which represents the predicted score (usually defined as probabilities, within $[0,1]$) that a classifier outputs for each instance. 

% % Regarding individual fairness metrics, the definition of the similarity might depend on a specific task~\cite{dwork2012fairness}, and it may be generally described as follows:

% % \begin{equation}
% %     |P[\hat{Y}_{i} = y | X_i, S_i] - P[\hat{Y}_j = y | X_j, S_j]| \le \epsilon;\;if\;d(i,j) \approx 0.
% % \label{eq:individual_fairness}
% % \end{equation}


% % \noindent
% % where $\hat{Y}_i$ is the model's prediction for individual $i$, $S_i$ refers to the sensitive attributes of individual $i$, and $X$ refers to his/her associated features. 
% % The distance metric $d(i,j)$ between individuals $i$ and $j$ can be defined depending on the domain, e.g., KL Divergence or L1-norm~\cite{biega2018equity}, and this is not a trivial task~\cite{pessach2020algorithmic}. 

% Different kinds of group fairness measurements have been proposed. 
% For example, \textit{demographic parity} (also known as \textit{statistical parity}) defines a fair classifier as one in which $\hat{Y}$ is independent of $S$~\cite{xu2020algorithmic}.
% Equivalently, it requires that the average of positive predictions be similar across different groups~\cite{calders2010three}. 
% % Formally, it is computed as:
% % \begin{equation}
% %     |P[\hat{Y} = 1 | S = 1] - P[\hat{Y} = 1 | S \neq 1]| \le \epsilon.
% % \label{eq:demographic_parity}
% % \end{equation}
% % \noindent
% % where $P$ is the probability, $\hat{Y}$ is the prediction, where $\hat{Y} = 1$ represents a positive prediction (e.g., acceptance of a specific condition, such as for a job). 
% % $S$ represents the protected attributes (e.g., race and gender), where $S = 1$ is the privileged group and $S \neq 1$ is the unprivileged group.
% % A lower value indicates more similar acceptance rates and thus more fairness. Intuitively, this metric tries to ensure that the positive prediction is assigned to the two sensitive groups at a similar rate. It is also independent of the ground-truth labels~\cite{du2020fairness}.
% Another example of group measure is \textit{equalized odds}~\cite{hardt2016equality}, which computes the difference between the false positive rates (FPR), and the difference between the true positive rates (TPR) of the two groups. It can be formalized as follows:

% \begin{equation}
%     |P[\hat{Y} = 1 | S = 1, Y = 1] - P[\hat{Y} = 1 | S \neq 1, Y = 1]| \le \epsilon,
% \label{eq:eq_odds_tpr}
% \end{equation}


% \begin{equation}
%     |P[\hat{Y} = 1 | S = 1, Y = 0] - P[\hat{Y} = 1 | S \neq 1, Y = 0]| \le \epsilon,
% \label{eq:eq_odds_fpr}
% \end{equation}


% \noindent
% where~\equref{eq:eq_odds_tpr} represents the absolute difference in the TPR of two groups bounded by $\epsilon$, and~\equref{eq:eq_odds_fpr} requires the absolute difference in the FPR of two groups to be bounded by $\epsilon$.
% Smaller difference between groups indicates better fairness. Since equalized odds relies on the actual ground truth (i.e., $Y$), it assumes that the base rates of the two groups are representative and were not obtained in a biased manner~\cite{pessach2020algorithmic}. 
% A less restricted metric, based on equalized odds, is \textit{equal opportunity}~\cite{hardt2016equality}, which requires only the true positive rates to be similar across groups,
% % The main difference is that if focuses on the true positive rates only
%  as in~\equref{eq:eq_odds_tpr}.

 
% % In our we use a slight variation of the definitions presented in~\eqref{eq:eq_odds_fpr} and in~\eqref{eq:eq_odds_tpr} based on the work of Xu et al.~\cite{xu2020algorithmic}.
% In our work we combine the definitions presented in~\equref{eq:eq_odds_fpr} and in~\equref{eq:eq_odds_tpr}, based on the work of~\cite{xu2020algorithmic}.
% Specifically, we use the metric $\Delta EO$, defined as the expectation of the absolute difference of true positive rate and false positive rate across two groups $S$.

% \begin{equation}
% \begin{split}
%     \Delta EO =|P[\hat{Y} = 1 | S = 1, Y = 0] - P[\hat{Y} = 1 | S \neq 1, Y = 0]| \\
%     +\;|P[\hat{Y} = 1 | S = 1, Y = 1] - P[\hat{Y} = 1 | S \neq 1, Y = 1]|.
% \end{split}
% \label{eq:delta_eo}
% \end{equation}




% % \begin{equation}
% %     |P[\hat{Y} = 1 | S = 1, Y = 1] - P[\hat{Y} = 1 | S \neq 1, Y = 1]| \le \epsilon,
% % \end{equation}
% % \label{eq:eq_opp_tpr}

% Some work have shown that it is not possible to simultaneously satisfy several metrics (notions) of fairness~\cite{corbett2017algorithmic, berk2018fairness, chouldechova2017fair, friedler2016possibility, corbett2018measure}. 
% Additionally, the literature discusses an existent trade-off between accuracy and fairness - as one increase fairness, it is possible to compromise accuracy~\cite{corbett2017algorithmic, kleinberg2016inherent}. 
% Overall, the goal of mitigating unfairness in algorithms is to achieve a model that allows for higher fairness without significantly compromising the accuracy or other alternative notions of utility.

% \subsection{Dataset}
% \label{subsec:dataset}

% In this work, we use the CelebA dataset~\cite{liu2015faceattributes}, which is a well-known benchmark in the ML community~\cite{shen2017learning, heusel2017gans, choi2018stargan}.
% Additionally, fairness issues within this dataset have been already studied by previous work~\cite{ramaswamy2021fair, sattigeri2019fairness, quadrianto2019discovering}.
% It contains celebrity faces with $40$ binary face attributes, corresponding to the presence ($1$) or absence ($-1$) of each facial trait.
% Each attribute was annotated by a ``professional labeling company'', further described by~\cite{bohlen2017server} as ``a group of $50$ paid male and female participants, aged $20$ and $30$, and recruited from mainland China during a $3$ month development phase''~\cite{sattigeri2019fairness}.
% It contains a total of $202,599$ images downloaded from the internet, cropped and resized to $128 \times 128$ pixels~\cite{denton2019image}.


==> sections/ack.tex <==
% \section*{Acknowledgments}
% \label{sec:ack}

% The authors would like to thank CNPq and CAPES for partially funding this work.
